Proving Unrealizability for Syntax-Guided Synthesis

Proving Unrealizability for Syntax-Guided Synthesis We consider the problem of automatically establishing that a given syntax-guided-synthesis (SyGuS) problem is unrealizable (i.e., has no solution). Existing techniques have quite limited ability to establish unrealizability for general SyGuS instances in which the grammar describing the search space contains infinitely many programs. By encoding the synthesis problem's grammar G as a nondeterministic program P_G, we reduce the unrealizability problem to a reachability problem such that, if a standard program-analysis tool can establish that a certain assertion in P_G always holds, then the synthesis problem is unrealizable. Our method can be used to augment any existing SyGus tool so that it can establish that a successfully synthesized program q is optimal with respect to some syntactic cost -- e.g., q has the fewest possible if-then-else operators. Using known techniques, grammar G can be automatically transformed to generate exactly all programs with lower cost than q -- e.g., fewer conditional expressions. Our algorithm can then be applied to show that the resulting synthesis problem is unrealizable. We implemented the proposed technique in a tool called NOPE. NOPE can prove unrealizability for 59/134 variants of existing linear-integer-arithmetic SyGus benchmarks, whereas all existing SyGus solvers lack the ability to prove that these benchmarks are unrealizable, and time out on them.

==> background.tex <==
\section{Background}
\subsection{Regular Tree Grammar}
\begin{definition}
	A regular tree grammar $G$ is defined by the tuple $(N,\Sigma,S,\delta)$ where
	\begin{itemize}
\item $N$ is a finite set of nonterminals,
\item $\Sigma$ is a ranked alphabet, i.e., an alphabet whose symbol have an associated their arities.
\item $S\in N$ is the starting nonterminals
\item $\delta$ is a finite set of productions of the form $A\to t(B_1,\cdots,B_k)$ with $A,B_1,...,B_k\in N$ and $t\in \Sigma^{(k)}$, or $A\to a$ with $A\in N$ and $a\in\Sigma^{(0)}.$
	\end{itemize}
\end{definition}

In this paper, we focus on \emph{typed} regular tree grammar where each nonterminal and each character  are associated with their types.

\subsection{Syntax Guided Synthesis}
Syntax guided synthesis is a formulation of program synthesis whose goal is finding a program in some candidate space that meets a correctness specification.
\begin{definition}[\sygus]
	A \sygus problem  is a tuple $(T,f,G,\varphi)$ where:
	\begin{itemize}
		\item $T$ is a background theory.
		\item $f$ is a symbol representing the synthesized function.
		\item $G$ is a typed regular tree grammar that only containing terms in $T$--i.e., $L(G)\subseteq T$.
		\item $\varphi$ is a Boolean formula built from the symbols in the background theory along with $f$.
	\end{itemize} 
	A solution of a \sygus problem $(T,f,G,\varphi)$ is an implementation $e\in L(G)$ for the function $f$ such that $\forall \overline{x}.\varphi(\overline{x})[f \leftarrow e]$ is valid.
\end{definition}We say a \sygus problem is \emph{realizable} if a valid solution exists, i.e., 
\begin{equation}
	\exists e\in L(G)\forall\overline{x}.\varphi(\overline{x})[f \leftarrow e].
	\label{eq:sygus}
\end{equation}
Similarly, a \sygus problem is \emph{unrealizable}--there exists no valid solution--iff
\begin{equation}
\forall e\in L(G) \exists \overline{x}.\neg\varphi(\overline{x})[f\leftarrow e].
\label{eq:unrealizable}
\end{equation}

\subsection{Reachability Verification Problem}

A \emph{program} $P$ takes an initial state $I$ as input and outputs a final state $O$, i.e., $\sem{P}(I)=O$ where $\sem{\cdot}$ is the semantic of programs as expected. In this paper, we allow programs contain calls to an external function \nd{} which returns non-deterministic Boolean values. When a program $P$ contains calls to \nd{}, we denote $P_{\nd{}}$ which is the same as $P$ except for that $P_{\nd{}}$ take an additional integer input $n$ and each call $\nd{}$ is substituted with a call to a local function \nextbit{} whose definition is:
$$\texttt{bool nextbit()\{bool b = n\%2; n=n>>1; return b;\}}.$$
That is, the integer $n$ instantiate all non-deterministic behavior of $P$ in $P_{\nd{}}$ by substituting non-deterministic values in $P$ with the next-bit of $n$ starting from the least significant bit.

For brevity, we denote $P^n(O)\eqdef P_{\nd{}}(n,O)$

\begin{example}
	\heping{example shows how $n$ determine the terms}
\end{example} 

The assertions are Boolean expressions over two states $I$ and $O$, which can be specified by Boolean functions $\assert{I,O}$.


\begin{definition}[Reachability Problem]
	A reachability problem is a tuple $(P,\assert{},I)$ where:
	\begin{itemize}
		\item $P:\mathcal{I}\to\mathcal{O}$ is a program containing non-deterministic branch.
		\item \assert{} is a Boolean function over $\mathcal{I}\times\mathcal{O}$.
		\item $I\in \mathcal{I}$ is a state in the input space. 
	\end{itemize}
The goal of a reachability problem is to determine the validity of the formula 
\begin{equation}
	\exists n.\assert{$I$,$\sem{P_n}(I)$}.
	\label{eq:reachability}
\end{equation}
\end{definition}

\subsection{Counterexample Guided Inductive Synthesis}
The CounterExample-Guided Inductive Synthesis (CEGIS) is a popular synthesis approach. Given the correctness specification $\forall x.\varphi(P,x)$, a CEGIS process consists of three components--a synthesizer $S$, a verifier $V$ and a counterexample set $\cex$--and two phases:
\begin{enumerate}
	\item call the synthesizer $S$ to find a candidate solution $P$ such that $\forall x\in\cex.\varphi(P,x)$ and go to phase 2; return \emph{unrealizable} if no candidate found.
	\item call the verifier $V$ to find a model $\mathcal{M}$ for query $\neg \varphi(P,x)$ and add $\mathcal{M}$ to $\cex$; return $P$ as a valid solution if no model found.
\end{enumerate}

Note that for \sygus problems, the CEGIS technique are usually used to only find a solution but not prove unrealizability since the candidate space is infinite.
However, our technique reformulate  synthesize problems as reachability problems such that we can use CEGIS to prove unrealizability.


==> conclusion.tex <==
% -*- TeX-master: t; TeX-PDF-mode: t -*-

\section{Conclusion}
\label{Se:Conclusion}

We presented a general technique for proving unrealizability of \sygus
problems.
Our technique encodes a synthesis problem's grammar $G$
and a given finite set of input examples $E$ as a
nondeterministic recursive program $\pge{G}{E}$ for which
(i) there is a path in $\pge{G}{E}$ corresponding to
each expression-tree generated by $G$, and
(ii) if a certain point in $\pge{G}{E}$ is unreachable, then the synthesis problem
is unrealizable.

We implemented the technique in a tool \name, which uses the program-analysis tool
SeaHorn to check reachability.
\name can automatically prove unrealizability for $\numSolved/\numBenchmarks$ unrealizable variants
of problems obtained from the \sygus-competition benchmark set.
\loris{discuss limitations}
    
%\rone \emph{natural}: requires minimal modification to the \sygus format,
%\rtwo \emph{general}:  it supports complex but practical types of weights,
%\rthree \emph{formal}: it is grounded in the theory of weighted tree grammars,
%\rfour \emph{effective}: our tool \name can solve quantitative variations of existing \sygus
%benchmarks with little overhead.
%%In our experiments, \name cannot solve some benchmarks  because
%%it reduces \qsygus problems  to multiple complex \sygus ones. 
%%However, we believe that, thanks to this new
%%application of \sygus solvers, our
%%new framework and synthesis technique will drive the design of existing \sygus solvers
%%to address the new challenging benchmarks that arise when solving \qsygus problems.
%In the future, we plan to extend our framework to handle 
% probabilistic objectives and
%quantitative objectives over the
%semantics of the program---e.g., synthesize programs that satisfy most of the specification.

%\mypar{Acknowledgements}
% This work was supported, in part,
% by a gift from Rajiv and Ritu Batra;
% by AFRL under DARPA MUSE award FA8750-14-2-0270 and DARPA STAC award FA8750-15-C-0082;
% by ONR under grant N00014-17-1-2889;
% by NSF under grants CCF-1637516 and CCF-1704117;
% by a Google Research Award;
% and by the UW-Madison Office of the Vice Chancellor for
% Research and Graduate Education with funding from the Wisconsin Alumni
% Research Foundation.
% Any opinions, findings, and conclusions or recommendations
% expressed in this publication are those of the authors,
% and do not necessarily reflect the views of the sponsoring
% agencies.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End: 


==> totalvsSeahorn.tex <==
\pgfplotsset{every axis/.append 
style={	
label style={font=\scriptsize}, 
tick label style={font=\scriptsize}}
}
\begin{figure}[!t]
\centering
\hspace{-2mm}
\begin{tikzpicture}[scale=1]
\begin{axis}[%
ymode=log,
xmode=log,
ylabel absolute, ylabel style={yshift=-3mm},
xlabel absolute, xlabel style={yshift=1mm},
width=.75\linewidth,
height=.525\textwidth,
scatter/classes={%
a={mark=*,draw=black,
mark options={solid},
mark size = 0.5}},
xmin = 0,
xmax = 400,
ymin = 0,
ymax = 400]
\addplot[scatter,only marks,%
scatter src=explicit symbolic]%
table {
x y 
1.48		0.53
58.57		50.21

0.69		0.17
0.87		0.21
101.44		87.92
134.87		118.77


112.78		87.32


1.12		0.38

0.43		0.18
0.49		0.19
0.46		0.17
0.58		0.18

0.38		0.11
1.56		0.54
11.32		5.68

1.28		0.72
9.16		6.98

369.57		361.21
};
%\addplot+[line width=1pt,mark size=.5pt] coordinates {(0,0) (300000,300000)};
%\addplot[color=red] coordinates { (1,0) (3,1) (6, 3) (9, 9) (10,15) (11,25) (12,40) (13, 60) (14,85) (16,140) (20,250)(21,280) (22,320)};
%\node [below, xshift=-1ex] at (axis cs:25.69,500) {\small TO};
\end{axis}
\end{tikzpicture}
\caption{The total solving time vs.\ solving time of \seahorn}
\label{fig:totalvsseahorn}
\end{figure}

